Client-side Vulnerabilities in Commercial VPNs

Internet users increasingly rely on commercial virtual private network (VPN) services to protect their security and privacy. The VPN services route the client's traffic over an encrypted tunnel to a VPN gateway in the cloud. Thus, they hide the client's real IP address from online services, and they also shield the user's connections from perceived threats in the access networks. In this paper, we study the security of such commercial VPN services. The focus is on how the client applications set up VPN tunnels, and how the service providers instruct users to configure generic client software. We analyze common VPN protocols and implementations on Windows, macOS and Ubuntu. We find that the VPN clients have various configuration flaws, which an attacker can exploit to strip off traffic encryption or to bypass authentication of the VPN gateway. In some cases, the attacker can also steal the VPN user's username and password. We suggest ways to mitigate each of the discovered vulnerabilities.

==> content/motivation.tex <==
%!TEX root = ../main.tex

\section{Motivation}
\label{sec:motivation}

Many users rely on the VPNs to protect their privacy, or in some cases to achieve anonymity. Despite the bold promises made by commercial VPN vendors, research has repeatedly shown that achieving complete privacy, let alone anonymity, over VPNs is a challenging task. Platform-specific surveys to study commercial~\cite{khan2018empirical}, industrial~\cite{rahimi2012analysis} and mobile VPNs~\cite{ikram2016analysis} has demonstrated a wide range of security and privacy vulnerabilities, such as DNS manipulation, traffic monitoring and leakage, sharing of the VPN infrastructure by multiple service providers.
%To our best knowledge, the vulnerabilities that we presented in this paper have not been discussed before in research literature.

It is evident from the plethora of research literature (refer to Section~\ref{sec:related}) that VPNs as a technology has undergone severe scrutiny to expose intentional malpractices by commercial VPN providers or other cryptographic vulnerabilities. Nonetheless, to our best knowledge, only a handful of them have taken a closer look into the client configurations of the commercial VPNs. More specifically, research conducted by Petra et al.~\cite{perta2015glance} demonstrates sophisticated DNS and IPV6 leakages, and the work by Rossberg et al.~\cite{rossberg2011survey} surveys problems with auto-configuration settings of commercial VPN clients. Our work extends this theme in the literature, and we believe that looking for additional flaws in VPN clients of commercial VPNs are non-trivial. Moreover, many commercial VPN service providers still support VPN protocols that are known to have insecure client configurations, such as with L2TP/IPSec, one of the widely used VPN protocols, has been known since 2016~\cite{l2tpkeys}. However, this issue has not been documented in research literature.


%%%%%%%%%%%%%%%%%%%%%%%%%%


Layer 2 Tunneling Protocol (L2TP)~\cite{townsley1999layer}, as its name suggests, is a tunneling protocol that operates on the data-link layer. Since L2TP itself includes no encryption or integrity protection for user data, it is often paired with IPsec \cite{atkinson1998security} to provide secure transport. The communicating nodes authenticate each other with a selected IKEv1 authentication method~\cite{harkins1998internet,maughan1998internet,piper1998internet}, such as a pre-shared keys based on the IP address of the client.  IKEv1 and the entire IPsec architecture reside in the IP layer, and thus, the IP address is the only clue available for them about the client identity. Since the clients of the commercial VPN services practically always have  dynamic IP addresses, it is not possible for the VPN gateway to support client-specific pre-shared keys. Obviously, the only option is to use the same key for all users, which is either publicly available online or can be discovered by looking at their client configuration. An example value of such pre-shared keys is ``12345678''.


As L2TP by itself does not provide any transport protection, the security of a L2TP/IPsec connection relies largely on the IPsec tunnel. However, since the network attacker knows the pre-shared key, it can perform a MitM attack to compromise the integrity and confidentiality of the connection. In addition, L2TP performs user authentication based on either the Password Authentication Protocol (PAP) or Challenge-Handshake Authentication Protocol (CHAP)~\cite{lloyd1992ppp}. With CHAP, the MitM attacker can pass the authentication messages between the honest server and honest client. On the other hand, if the authentication uses PAP, the attacker will also capture the victim's VPN ID and password. In any case, the MitM attacker is able to decrypt all the network traffic from and to the victim's computer.

\sr{I feel, it is good to somehow retain this paragraph. But, I am not sure how to do it without having the previous tech heavy paragraph}.
At this point, it is worth discussing the reason for the use of fixed keys in L2TP/IPsec.  On one hand, there have been proprietary proposals for sending a hint about the client identity to the server, but the rather historical IKEv1 protocol and its implementations have not been updated to support such new features in an interoperable way. Thus, the commercial VPN services have fallen back to the insecure practice of sharing the same key between all clients. On the other hand, switching from pre-shared keys to certificate authentication would solve the problem. However, this would be an administrative hurdle for the VPN service providers, and might scare away non-expert customers. Thus, the service providers have opted to continue the insecure services rather than endanger their business growth. 

In spite of its known insecurity and availability of solutions, as we confirmed from our initial analysis, most of the popular commercial VPN services have not fixed the issue with L2TP/IPSec. whether the reason is the reliance on legacy technology or business decisions, such security flaws remain opaque to the end-users. Especially since commercial VPNs are sold as a privacy-enhancing technology to general public, rather than a remote access commodity for technically-savvy people. In this realm, we feel that it is important to further the research, specifically by re-scrutinizing the VPN client configurations, which otherwise would undermine the privacy of regular Internet users. \sr{initial lines from Threat Model or something about goals can go here}.


%%%%%%%%%%%% Text to edit for discussion 

For example, the issue of using publicly known pre-shared keys for L2TP/IPsec has been known since 2016, but it has not been addressed by any of the commercial VPN services. %\sr{move to motivation section - For example, the issue of using publicly known pre-shared keys for L2TP/IPsec has been known since 2016, but it has not been addressed by any of the commercial VPN services. This issue could be solved by provisioning certificates to the clients, but that would be an administrative hurdle for the VPN service provides and might scare away non-expert customers. Thus, the service providers have opted to continue the insecure services rather than endanger their business growth.}


It is worth discussing the reason for the use of fixed keys in L2TP/IPsec and Cisco VPN. In the IKEv1 Main Mode, the server selects the pre-shared key by the IP address of the client. IKEv1 and the entire IPsec architecture reside in the IP layer, and thus, the IP address is the only clue available for them about the client identity. Since the clients of the commercial VPN services practically always have  dynamic IP addresses, it is not possible for the VPN gateway to support client-specific pre-shared keys. There have been proprietary proposals for sending a hint about the client identity to the server, but the rather historical IKEv1 protocol and its implementations have not been updated to support such new features in an interoperable way. Thus, the commercial VPN services have fallen back to the insecure practice of sharing the same key between all clients.

